Determining the Optimal Frequencies for a Duplicated Randomized Clock SCA Countermeasure

Side-channel attacks pose significant challenges to the security of embedded systems, often allowing attackers to circumvent encryption algorithms in minutes compared to the trillions of years required for brute-force attacks. To mitigate these vulnerabilities, various countermeasures have been developed. This study focuses on two specific countermeasures: randomization of the encryption algorithm's clock and the incorporation of a dummy core to disguise power traces. The objective of this research is to identify the optimal frequencies that yield the highest level of randomness when these two countermeasures are combined. By investigating the interplay between clock randomization and the presence of dummy cores, we aim to enhance the overall security of embedded systems. The insights gained from this study will contribute to the development of more robust countermeasures against side-channel attacks, bolstering the protection of sensitive information and systems. To achieve this, we conduct simulations and perform side-channel attacks on an FPGA to establish the relationship between frequencies and the resulting protection. We break the encryption on a non-duplicated circuit and note the least amount of measured power traces necessary and the timing overhead. We do this for all sets of frequencies considered which gives a good indication of which sets of frequencies give good protection. By comparing the frequencies generated with those from the duplicated circuit we use similar conclusions to prove whether a frequency set is secure or not. Based on our results we argue that having one frequency lower than half of the base frequency and the other frequencies being close but not higher than the base gives the highest security compared to the timing overhead measured.

==> Figures/Sim_results.tex <==
\begin{table}[H]
\centering
{\footnotesize
\begin{tabular}{| p{1.6cm} | >{\scriptsize \centering}p{1.6cm}|p{6cm}|  p{1.2cm} | p{1cm}|}
\hline
\multicolumn{5}{|c|}{Simulated frequencies} \\
\hline
Frequency group &  {\footnotesize Frequencies (MHz)} & Graph &    Nr. freqs &  Unique freqs\\
\hline
Previous work &  $f_{base}$=10 $f_1$=11.9713 $f_2$=7.7315 $f_3$=9.2778  $f_4$=12.6515 & \raisebox{-\totalheight} {\includegraphics[width=60mm, height=30mm]{Images/Single/Default.png}} & 77745 &  412  \\
\hline
Two low, one above half, one lower than half &   $f_{base}$=10 $f_1$=9.5917 $f_2$=9.0317 $f_3$=6.2777 $f_4$=4.0517 & \raisebox{-\totalheight} {\includegraphics[width=60mm, height=30mm]{Images/Single/cl10, 9.5917, 9.0317, 6.2777, 4.0517.png}} & 28610 & 458 \\
\hline
Two high, two lower than half &   $f_{base}$=10 $f_1$=3.6719 $f_2$=4.4021 $f_3$=12.9781 $f_4$=14.4317 & \raisebox{-\totalheight} {\includegraphics[width=60mm, height=30mm]{Images/Single/cl10.0, 3.6719, 4.4021, 12.9781, 14.4317.png}} & 33992 & 502\\
\hline
Three high, one lower than half &   $f_{base}$=10 $f_1$=4.7717 $f_2$=11.5019 $f_3$=12.0779 $f_4$=13.5319 & \raisebox{-\totalheight} {\includegraphics[width=60mm, height=30mm]{Images/Single/cl10.0, 4.7717, 11.5019, 12.0779, 13.5319.png}} & 38910 & 496\\
\hline
Three low, one lower than half &   $f_{base}$=10 $f_1$=9.1942 $f_2$=9.2708 $f_3$=9.9330 $f_4$=4.3457 & \raisebox{-\totalheight} {\includegraphics[width=60mm, height=30mm]{Images/Single/cl10.0, 9.2003, 9.3001, 9.4001, 4.4003.png}} & 30796 & 458\\
\hline
Three high, one above half &  $f_{base}$=10 $f_1$=5.9009 $f_2$=11.5019 $f_3$=12.0779 $f_4$=13.5319 & \raisebox{-\totalheight} {\includegraphics[width=60mm, height=30mm]{Images/Single/cl10.0, 5.9009, 11.5019, 12.0779, 13.5319.png}} & 39929 & 468\\
\hline

\end{tabular}

\clearpage

\begin{tabular}{| p{1.6cm} | >{\scriptsize \centering}p{1.6cm}|p{6cm}|  p{1.2cm} | p{1cm}|}

\hline
Three low, one lower than half &   $f_{base}$=10 $f_1$=9.1942 $f_2$=9.2708 $f_3$=9.9330 $f_4$=4.3457 & \raisebox{-\totalheight} {\includegraphics[width=60mm, height=30mm]{Images/Single/cl10.0, 9.2003, 9.3001, 9.4001, 4.4003.png}} & 30796 & 458\\
\hline
Three high, one above half &  $f_{base}$=10 $f_1$=5.9009 $f_2$=11.5019 $f_3$=12.0779 $f_4$=13.5319 & \raisebox{-\totalheight} {\includegraphics[width=60mm, height=30mm]{Images/Single/cl10.0, 5.9009, 11.5019, 12.0779, 13.5319.png}} & 39929 & 468\\
\hline

\end{tabular}
}
\caption{Frequency test on hardware}

{\footnotesize The frequencies generated by all sets of input frequencies are displayed in this table. Each row contains one set of frequencies and has the total number of frequencies generated as well as the number of unique frequencies. The first column represents the relation between the frequencies and the base frequency.}
\label{tab:simulation_results}
\end{table}

==> Figures/randomVSnonerandom.tex <==
\begin{figure}
  \begin{subfigure}{0.5\textwidth}
    
    \includegraphics[width=\linewidth]{Images/Single/NonRandomAES.png}
   
    \caption{\centering The first/last round of AES is easy to find with a none randomized clock.}
  \end{subfigure}%
  \begin{subfigure}{0.5\textwidth}
    
    \includegraphics[width=\linewidth]{Images/Single/RandomAES.png}
    \caption{\centering 10 Captured power traces with randomized clock.}
  \end{subfigure}
  \caption{\centering Shows the difficulty of processing several randomized traces compared to none randomized traces.  }
  \label{figure:randomVSnonerandom}
\end{figure}
